3D-IntPhys: Towards More Generalized 3D-grounded Visual Intuitive Physics under Challenging Scenes

Given a visual scene, humans have strong intuitions about how a scene can evolve over time under given actions. The intuition, often termed visual intuitive physics, is a critical ability that allows us to make effective plans to manipulate the scene to achieve desired outcomes without relying on extensive trial and error. In this paper, we present a framework capable of learning 3D-grounded visual intuitive physics models from videos of complex scenes with fluids. Our method is composed of a conditional Neural Radiance Field (NeRF)-style visual frontend and a 3D point-based dynamics prediction backend, using which we can impose strong relational and structural inductive bias to capture the structure of the underlying environment. Unlike existing intuitive point-based dynamics works that rely on the supervision of dense point trajectory from simulators, we relax the requirements and only assume access to multi-view RGB images and (imperfect) instance masks acquired using color prior. This enables the proposed model to handle scenarios where accurate point estimation and tracking are hard or impossible. We generate datasets including three challenging scenarios involving fluid, granular materials, and rigid objects in the simulation. The datasets do not include any dense particle information so most previous 3D-based intuitive physics pipelines can barely deal with that. We show our model can make long-horizon future predictions by learning from raw images and significantly outperforms models that do not employ an explicit 3D representation space. We also show that once trained, our model can achieve strong generalization in complex scenarios under extrapolate settings.

==> figText/visual_head_bar.tex <==
\begin{figure}[t!]
    \vspace{-5pt}
    \centering
    \includegraphics[width=.99\linewidth]{imgs/results/visual_head_bar_v1.pdf}
    \vspace{-8pt}
    \caption{\small
    \textbf{Quantitative Results of the Perception Module.}
    \yl{need to change to table.}
    We compare our method with two baselines: autoencoder (AE) and NeRF-dy~\citep{nerf-dy}. The \textcolor{blue}{blue} bar shows the mean squared error (MSE) between the reconstructed image and the ground truth (lower is better). The \textcolor{red}{red} bar indicates the structural similarity index measure (SSIM) of the prediction (higher is better).
    %
    Our method performs the best across all metrics and has shown huge improvements especially in extrapolate settings.
    % Quantitative analysis of visual head reconstruction, three methods(ae, nerf-dy, ours) are compared using two metrics: Mean Squared Error (MSE) and Structural Similarity (SSIM) \hth{Make x-axis font as big as possible, x-axis labels will merge into each other if font is too big}
    }
   \label{fig:visual_head_bar}
   \vspace{-10pt}
\end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> text/checklist.tex <==
\section*{Checklist}


\begin{comment}
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\end{comment}


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}. We have included limitations of the proposed work in Section \ref{sec:conclusion}.
  \item Did you discuss any potential negative societal impacts of your work?
   \answerYes{} We have included the discuss in the supplementary material.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
   \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}  Please see the paragraph ``implementation details'' in Section \ref{sec:exp} and the supplementary material for the details.
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}. We have illustrated standard deviation in Figure~\ref{fig:dynamics_curve}.
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} The details are provided in the supplementary material.
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
   \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
   \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
   \answerNA{}
\end{enumerate}


\end{enumerate}



==> text/experiments_v1.tex <==
\section{Experiments}

\input{figText/dataset.tex}

\subsection{Datasets}
We generated three local varied simulation datasets using physics simulator Nvidia Flex \cite{flex}. Each of the dataset represents one specific kind of manipulation scenario like Pouring, Shaking and Pushing, which are three basic manipulations in our everyday life. For each of the three scenarios, we change some properties of objects in the scene, e.g. the shape of container, the amount of water, the color/number of cubes to make it diverse, as we can see in Figure \ref{dataset}. To test the generalization capability of the trained model, we use unseen settings of each scenario in test stage. More settings and samples of the dataset can be referred to in Appendix \ref{appendix-dataset}.

\paragraph{FluidPour} This environment contains a fully-actuated cup pouring colored fluids into a container on the plane. We  use different shapes of container, number of water fluids, different pouring actions test the generalization of the model.

\paragraph{FluidCubeShake} This environment contains fully-actuated container
moves on a 2D plane. Inside the container there are colored fluids and colored cubes. We  use different shapes of container, number of cubes, color of cubes different shaking actions test the generalization of the model.

\paragraph{GranularPush} This environment contains fully-actuated board that is pushing a granular cube. Here we tried different amount of initialized granular to test the generalization of the model.

\subsection{Baseline Methods and Evaluation Metrics}

Learning visual dynamics from fluid scenes is challenging, here we try to compare our method with recently proposed Nerf-dy \cite{nerf-dy}. Nerf-dy is also the first 3-D aware framework that can learn intuitive physics from multi-view videos, which is proved to outperform methods that directly apply autoencoder to encode 3-D scenes. Nerf-dy also benefits from NeRF structure on its visual perception head. We make this comparison in all of the three datasets for particle-based long-time rolling prediction.

We also do experiments on visual reconstruction head on Auto Encoder-based reconstruction without 3-D aware information and compare the reconstruction performance of all three methods, and here we name them AutoEncoder(AE), Nerf-dy and our method(Ours).  We make the comparison based on the Mean Squared Error (MSE) and Structural Similarity (SSIM) in pixel level (Fig. \ref{visual_head_bar}).


% The evaluation of the learned visual dynamics model focuses on three dimensions: (1) Performance on the three datasets which are correlated to three basic operations on fluid or granular object: Pour, Shake and Push. (2) Performance of dynamics model on different rolling scales (e.g. 50-frames short time rolling, 200-frames long time rolling). (3) The generalization ability of the model on interpolate and extrapolate testing environments.





\input{figText/visual_head_bar}
\input{figText/visual_head}

\input{figText/exp_dynamics}
\input{figText/dynamics_curve}



\subsection{Results}

The evaluation of the learned visual dynamics model focuses on three dimensions: (1) Can we get a good intermediate visual
reconstruction from the visual head of the visual intuitive physics learners to be evaluated? (2) Can the models to be evaluated work on scenes with Fluids, Rigid Objects and Granular Materials respectively ? (3) Can the evaluated models generalize to learn generalized 3-D intuitive physics regarding long-time rolling prediction in extrapolate settings?

\paragraph{Learning from complex dynamics scenes}
It is challenging to learn visual dynamics without additional annotations for scenes with Fluids, Rigid Objects and Granular Materials. Here we focus on learning 3-D visual dynamics and we will compare our 3D-IntPhys model with Nerf-dy. We test them on the three datasets mentioned above : \textbf{FluidPour}, \textbf{FluidCubeShake} and \textbf{GranularPush}. From qualitative results in Fig. \ref{exp_dynamics} we can see that, Nerf-dy can learn relatively reasonable movement of Fluids, but failed in learning dynamics of Cubes and Granular Materials. Our 3D-IntPhys can learn  reasonable dynamics from all of the three kind of scenes. This gap is caused by the strong inductive bias in both the visual head and dynamics head, where our model can fetch more 3-D information from the visual inputs and learn garph-based dynamics model.

\paragraph{Visual Head Reconstruction}
Also, it is important for visual dynamics model to learn well-performed visual perception module. This is of great importance when analyzing the two-stage visual intuitive learner. We will compare the visual head reconstruction results of our 3D-IntPhys with that of traditional AutoEncoder structure and visual head of Nerf-dy. We find that the visual head of our model can get much better reconstruction in all the three environments than the other two methods (Fig. \ref{visual_head}). A Our method also outperforms the other two methods, especially in \textbf{FluidCubeShake} and \textbf{GranularPush} in quantitative analysis in Fig. \ref{visual_head_bar}.

\paragraph{Generalization on different settings}

We also work on testing the if the visual intuitive learned by our model can generalize on both interpolate and extrapolate settings. We increase the diversity of the dataset by bring into different settings (e.g. Fluids Amount, Cube Color, Cube Number, Granular Materials Amount). Moreover, at testing stage, we introduce extrapolate settings of all of the three environments respectively which are unseen at training stage. We find that our model can well-generalized to extrapolate settings both at visual perception stage and dynamics learning stage. Nerf-dy and AutoEncoder cannot generalize well at visual head under extrapolate settings.For \textbf{FluidShake}, they cannot catch the color information of rigid cubes (Fig. \ref{visual_head}). For Nerf-dy, its gap between interpolate and extrapolate settings is bigger, and it fails to learn dynamics of rigid objects and granular materials in extrapolate settings. 


% We test the visual head for each of the three models, since our model and Nerf-dy are 3D-aware and AutoEncoder is not, we use  Mean Squared Error (MSE) and Structural Similarity(SSIM) to determine the quality of visual head outputs. From both qualititive results (Fig. \ref{visual_head_bar}) and quantitative results (Fig. \ref{visual_head}), we can see that, 3-D aware methods are better than AutoEncoder, which is accordance with findings in \cite{nerf-dy}. Also, our model outperforms Nerf-dy in all three environments and the gap is bigger with the increase of diversity of the scene.

% Also, we compare the results of long-time rolling prediction in 3-D space between our model and Nerf-dy. We sample the predicted frames in 3-D space and visualize it by taking pictures from a specific angle (Fig. \ref{exp_dynamics}). Also we sample from both interpolate and extrapolate settings and calculate the prediction loss based on Chamfer Distance between predicted point cloud state and ground truth state. Here we should note that, since we cannot accurately segment cubes from Nerf-dy point cloud using color information, we just ignore cubes in the qualitative analysis. The qualitative curve can be referred to in  Fig. \ref{dynamics_curve}. From these results, we can see that our model can generalize well under extrapolate settings and performs better than Nerf-dy in long-time prediction, especially in most complex scenes like extrapolate settings of GranularPush. 


% From the results we can see that : though using only visual inputs and two steps of rolling prediction to train our model, we can still learn good long-time 3-D dynamics that are align with physics intuition. The results also show the privilege of our model in visual scenes with great diversity, considering both the ability of visual head perception and 3-D aware dynamics learning. Specifically, compared with Nerf-dy, our method can work better when we increase the diversity of the scene: Nerf-dy can work at most FluidPour scenes but fail at GranularPush scenes. 



 
% Here we focused on the dynamics prediction results learned from the video inputs of (1) (inside) Scenarios which are formed by objects in the training datasets (2) (outside) Scenarios which are formed by objects that have never shown up in the training datasets (e.g. container with new shapes, new amount of particles, new number/color of cubes).

% Here we use segmented IoU(SegIoU@K) to measure the accuracy of predicted results, where $K$ represents the rolling number, if a model can predict acceptable results after a longer rolling time with the accumulation of error and turbulence, the dynamics it learned is more robust . We first choose a suitable view direction, then for each method, we render the prediction result of interested ares in this view direction and compare them with the interested ares in the ground-truth. Mathematically, if there are $N$ interested area (e.g. fluids, cube, granular), the target areas in ground truth image taken from specific angle in rolling number $k$ can be decomposed into pixels of interested areas: $I^{k} = I_{1}^{k} \cup I_{2}^{k} ...\cup I_{N}^{k}$ based on color information. The predicted $n$ interested patches of pixel is $\hat{I}^{k} = \hat{I}_{1}^{k} \cup \hat{I}_{2}^{k} \cup ... \hat{I}_{N}^{k}$. 

% \begin{equation}
%     SegIoU@K = \frac{1}{KN}{}\sum_{k=1}^{K}\sum_{n=1}^{N}\frac{|I_{n}^{k} \cap \hat{I}_{n}^{k}|}{|I_{n}^{k} \cup \hat{I}_{n}^{k}|}
% \end{equation}

% Actually, for our methods, we can predict the 3D position of particle and compare them with the ground truth, which makes the learning process of the model more interpretable and controllable, since we can debug the visual and dynamics branch separately instead of combine them as an end-to-end black box. However, as far as our knowledge, there is no such methods that use explicit 3d particle representation to learn dynamics from video before. For fair comparison, the point cloud similarity can not be used to measure between our methods and previous methods. 

% \begin{table*}
% \centering
% \resizebox{\linewidth}{!}{ %< auto-adjusts font size to fill line
% \begin{tabular}{@{}lccccccccc@{}}
% \toprule
% Dataset & \multicolumn{3}{c}{FluidPour (seen/nseen)} & \multicolumn{3}{c}{FluidCubeShake (seen/nseen)} & \multicolumn{3}{c}{GranularPush (seen/nseen)} \\
% \midrule
% Methods & SegCD@50 \downarrow & SegCD@100\downarrow & SegCD@200\downarrow & SegCD@50 \downarrow& SegCD@100\downarrow & SegCD@200 \downarrow& SegCD@50\downarrow & SegCD@100\downarrow & SegCD@200\downarrow \\
% AE-dy & 0/0 & 0/0 & 0/0 & 0/0 & 0/0 & 0/0 & 0/0 & 0/0 & 0/0\\
% Nerf-dy & 0/0 & 0/0 & 0/0 & 0/0 & 0/0 & 0/0 & 0/0 & 0/0 & 0/0\\
% Ours & 0/0 & 0/0 & 0/0 & 0/0 & 0/0 & 0/0 & 0/0 & 0/0 & 0/0\\
% \bottomrule
% \end{tabular}
% } % \resizebox
% \caption{
% % 
% \textbf{Quantitative Results} -- Glory to the bold numbers.
% % 
% } % \caption
% \label{tab:sota}
% \end{table*}




==> text/method_v1.tex <==
\section{Methods}\label{model}

\input{figText/pipeline}

%gps: graph-based 
% unsupervised particle-bas
We present Visual Intuitive Phyisics Simulator (VIPS), a model that learns to 
VIPS contains a visual inference module that 

Here we will introduce our framework to learn dynamics model using unlabelled RGB images. The framework can be divided into two parts:
\begin{itemize}
    \item A visual front-end to generate 3D particle representation 
    \item A graph neural networks based dynamics learner to learn particle-based dynamics
\end{itemize}  

This framework decouples the visual-based dynamics learning process into two separate parts, which also aligns with human's learning style of intuitive physics: we first have a 3D understanding of the scene, that we try to learn the interaction between scene components. Also, this separation makes the whole pipeline more interpretable and easier to debug compared with methods using deep visual feature.

It should also be noted that both the visual and the dynamics branch is strongly generalized since they are all learned with local features, the visual branch takes the local feature of queried point in voxel space and the dynamics branch use graph to represent the scene where local relations are used to pass messages among the graph. 



\subsection{Generalized Neural Radiance Field for Dynamic Scenes Reconstruction}
The visual branch takes in sequential frames of RGB images taken from $N_v$ different views. For a specific trajectory in the dataset that contains $N_f$ frames, the input size is actually $[N_f , N_v ,H , W , 3]$ where the last three terms are resolution of input RBG images. What we want to reconstruct is sequence of point clouds sized $[N_f , N_p, 3]$, $N_p$ is the size for the point cloud of key object in the scene after using farthest point sampling, since the raw point cloud reconstructed is of huge size and is computationally expensive .

\paragraph{Nerual Radiance Field}  NeRF\cite{nerf} learns to reconstruct a volumetric radiance field of a scene given the 3D points $\textbf{x} \in \mathbb{R}^3$ and the view direction $\textbf{d}\in \mathbb{R}^3$ for each point.  It can be formulated as a function : 
$F_{\phi}(\textbf{x}, \textbf{d}) = (\textbf{c}, \sigma)$ where $\textbf{c}$ is the RGB color of the queried point and $\sigma$ is the corresponding density, which can be used to decide where there is a object component in the scene. 

The volumetric radiance field can then be rendered into a 2D image via $\hat{\textbf{C}}(\textbf{r})=\int_{t_n}^{t_f}T(t)\sigma(t)c(t)dt$, $T(t)=exp(-\int_{t_n}^{t}\sigma(s)ds)$ is used to calculate the occlusion. We then formulate a camera ray as $\textbf{r}(t) = \textbf{o}+h\textbf{d}$, where $o\in\mathbb{R}^3$ is the origin of ray and $d\in\mathbb{R}^3$ is a unit direction vector for the ray. The rendering range is controlled by the depths of the near, far plane $t_n$ and $t_f$. Then we can train NeRF by comparing our prediction RGB pixel in the camera plane with the ground-truth by:

\begin{equation}
    \mathcal{L} = \sum_{\textbf{r} \in \textbf{P}} \|\hat{\textbf{C}(\textbf{r})} - \textbf{C}(\textbf{r}) \| 
\end{equation}

where $\textbf{P}$ is all the camera rays sampled from different views.

The biggest limitation of traditional NeRF is that it cannot be generalized in different scenes. Since NeRF only use the position and view direction as inputs, we can only train one NeRF model for one specific scene. So we can not achieve a generalized visual branch for all different trajectories using traditional NeRF.

\paragraph{Image-conditioned NeRF.} Here we turn to a image-conditioned NeRF (pixelNeRF)\cite{pixelnerf} to strongly improves the generalization of NeRF which can be trained on images taken from different scenes and help with the reconstruction of our particle frames. The idea of pixelNeRF is to add more visual information of the queried point into the NeRF predictor. Given an image $\textbf{I}$ in a scene, pixelNeRF first extract a feature volume using a CNN encoder
$\textbf{W} = E(\textbf{I})$. For a  point $\textbf{x}$ in the world coordinate, we retrieve its feature vector by projecting it onto the image plane, so that we can get the feature vector $\textbf{W}(\pi(x))$. Then pixelNeRF combines the feature vector together with the geometry position of that point and predict the RGB color and density information: 
\begin{equation}
  \label{pixelnerf}
    F_{\phi}(x, \textbf{d}, \textbf{W}(\pi(x)) = (\textbf{c}, \sigma)
\end{equation}

Also, pixelNeRF can incorporate multiple views to help with generalization, since there is fewer ambiguity in more views. For a queried position $\textbf{x}$, pixelNeRF can get feature vectors retrieved from $N_v$ views, then it can compute the hidden states $\textbf{V}^{(i)}(\textbf{x})$ $(i \in \{1,2,3 ..., N_v\})$ using Equation \ref{pixelnerf}. The final color and density is predicted using the average pooling aggregation of hidden states of $N_v$ views: 
\begin{equation}
    (\sigma, \textbf{x}) = f(P(\textbf{V}^{(1)}, \textbf{V}^{(2)}, ..., \textbf{V}^{(N_v)}))
\end{equation}

The training procedure is the same as traditional NeRF using re-rendering loss compared with ground-truth RGB images. The pixel-NeRF can be greatly generalized since it take into account the visual features of the queried point from different views.

\paragraph{Particle representation  generated from trained pixelNeRF} For a dataset that contains $N_t$ trajectory videos, each video  has $N_f$ frames and each frame is taken from $N_v$ views. Actually we have $N_t * N_f * N_v$ images from $N_{s} = N_t * N_f$ different scenes. We note $\textbf{I}^{(i, j, k)}$ as the image from $i$-th trajectory, $j$-th frame and $k$-th view. We can train a pixelNeRF $F_{\phi}$ on the a subset of the trajectories and it can generalize in other trajectories.

Then for scene $s \in \{1, 2, ..., N_s\}$ with $O_s$ target object(such as fluid, cube), we sample a volumetric space $\textbf{R}(T)$ sized $T * T * T$ which can cover the scene and query all the $T^3$ points in the volume to get $(\textbf{c}, \sigma) = F_{\phi}(\textbf{R}(T))$. Then we can select from the $\textbf{R}(T)$ using the density value $\sigma$ to get the point cloud of objects in the scene(container, water, box, robot arm, table): $\textbf{R}_{obj}(T) = \{t \in \textbf{R}(T) | \sigma(t) > \sigma_{min}\}$, where $\sigma_{min}$ is the lowest bar for object density. Here we use color as prior information to segment out the particles we want to modeling(water, box). Specifically, for target particles which forms a object $o_{i} \in \{1, 2, 3, ..., O_s\}$, we can get the point cloud of this object: $\textbf{R}_{o_{i}}(T) =  \{t \in \textbf{R}_{obj}(T) | \textbf{c}(t) \in r(o_i)\}$ where $r(o_i)$ is the color set for object $o_i$. We note the final point cloud of scene $s$ as $p_{s} = \{p_{s}^{1}, p_{s}^{2}, ..., p_{s}^{O_s}\}$.

Then we can do sparse sampling of each point cloud using FPS (Farthest Point Sampling) \cite{fps}, which can sample small subset of the target point cloud and maintain the shape of it. To facilitate the learning of particle-based dynamics, we set the size after sampling fixed.



\subsection{Dynamics Modeling}
Dynamics modeling is a vital task in learning intuitive physics, it can also help with many tasks in robot learning like control and manipulation. The main idea of dynamics modeling is to predict the movement of particles in next frames using just a small number of history frames (e.g. using states of $\{v^{s - 5}, v^{s-4}, ..., v^s\}$ to predict states at $\{v^{s+1}, v^{s+2}, ..., v^{s+30}\}$) where $v^{i}$ is the state of the scene at time step $i$. The key idea of dynamics modeling used in this paper is decomposing the whole scene into particle-based objects. Then we use graph neural networks to do state encoding, message passing and movement prediction. Also, this kind of particle-based modeling can help us train generalized model that can also work in extrapolate environments when we add more particles into the system.


\paragraph{Build dynamic graph}
At each frame, the particle representation reconstructed by pixelNeRF is a point cloud which define the spatial span of target objects. We name $X$ as positions of particle, $G$ as group information to represent different object instances (e.g. fluid, container, cubes ...), and $Q$ as rigid properties of particles which determines whether the point belongs to a rigid body. Then we can form a graph $\langle V, E\rangle$ based on the distance between points. Each vertex $v_i=(\dot{x}_i, a_i^{v}) \in V$ contains the velocity of the point : $\dot{x_i}$ and particle attributes : $a_i^{v}$. For each relation $e_i \in E$, we have $e_i=(Rr_i, Rs_i, a_i^{e})$ where $Rr_{i}$ and $Rs_{i}$ are indices of receiver point and sender point and $a_i^{e}$ is attributes of relation to indicate the types of relation (e.g. collision, spring force).


\paragraph{Spatial message passing and propagation. }\label{dpi_dynamics}
Similar to traditional graph neural networks, at time step $t$, we can do message passing to update the state of representation of particles and relations in the scene:

\begin{equation}\label{relation_encode}
    g_{i, j}^t = Q_{r}(v_i^t, v_j^t, a_{ij}^{r})    ~~~~~~~~     (i, j) \in E
\end{equation}

\begin{equation}\label{relation_encode}
    h_{i}^t = Q_{v}(a_{i}^{e}, \sum_{k \in \mathcal{N}(i)}g_{i, k}^t)  ~~~~~~~~~~~~ i \in V
\end{equation}


$Q_v$ and $Q_r$ are encoders for vertices and relations respectively, $\mathcal{N}(i) = \{j|(i, j) \in E\}$. Though this kind of message passing can help with updating representation or passing of forces, it can only share one-hop information in each time step, which limits its performance on instantaneous passing of forces. So we can use multi-step message propagation in \cite{DPI} , for example we do $L$ steps of propagation, we reuse the notation $Q_r, Q_e$ mentioned above to encode particles and  relations, also we have $P_r, P_e$ to work as propagation function of particles and relations.


\begin{equation}
       \label{prop1}
    g_{r, t}^{l} = P_{r}(c^{r}_{r, t}, h^{l-1}_{j, t}, h^{l-1}_{j, t}), ~~~~ r=(i, j) \in E
\end{equation}

\begin{equation}
 \label{prop2}
    h_{i, t}^{l} = P_{e}(c^{e}_{i, t}, \sum_{k \in \mathcal{N}(i)}g_{(i, k), t}^{l}, h_{i, t}^{l-1}), ~~~~ i \in V
\end{equation}

The above formulation are propagation step $l \in \{0, 1, 2, ..., L\}$ in time step $t$, where $c^{r}_{r=(i, j), t}=Q_r(v_{i}^{t}, v_{j}^{t}, a^{t}_{ij})$, $c^{e}_{i, t} = Q_e(v_{i}^{t})$ is the encoded representation for particles and relations. $g_{r, t}^{l}$ is the effect of relation $r$ in propagation step $l$ and $h_{i, t}^{l}$ is the hidden states for each particle in propagation process. The propagation step $0$ is an initialization step where $h_{i, t}^{0} = \textbf{0}$ for all vertices. Finally we have the predicted states of particles at time step $t$ after $L$ steps of propagation:

\begin{equation}
    \hat{v}_{i}^{t+1} = f_{pred}(h_{i, t}^{L})
\end{equation}


\paragraph{Training dynamics model without particle-level correspondence}
Different from traditional dynamics model trained with dense trajectory information for each particles, our pipeline generate object-centric point clouds directly from RGB-images, so there does not exist an explicit one-to-one correspondence for particles in different frames. Especially for scenarios with fluid in it, it is hard to get the velocity of each particles. However, we can still train a dynamics predictor mentioned in \ref{dpi_dynamics}  with the help of ground-truth positions of some known objects like robot arms and containers. Intuitively, when we know the movement of cup, we can also predict the movement of water poured out by the cup.

More detailed approach of training dynamics model without particle-level correspondence between frames is discussed in Appendix \ref{dpi-wo-correspondece}.


After we make prediction based on history frames ($\{t_0, t_1, ..., t_h\}$), we get our predicted states on the $t_{h+1}$ frames, which is a point cloud: $\hat{P}^{t_{h+1}}=\{\hat{V}^{t_{h+1}}_i|i\in\{1, 2, ..., N_P\}\}$ where $N_P$ is the number of interested particles like fluid and cubes. The ground truth is also a point cloud $P^{t_{h+1}}$ sized $N_P$ but we do not have a one-to-one correspondence between $P^{t_{h+1}}$ and $\hat{P}^{t_{h+1}}$, which means we cannot use L-2 loss in particle level like many particle-based dynamics models do. Here we turn to a widely-used metric to calculate the similarity between two point clouds, which can be used as the loss function to train our dynamics model:

\paragraph{Chamfer Distance }
    The chamfer distance $d_c(P_1, P_2)$ between two point cloud $P_1$ and $P_2$ is defined as:
    \begin{equation}
    \setlength{\abovedisplayskip}{3pt}
    \setlength{\belowdisplayskip}{3pt}
    d_{c}(P1, P2) = \frac{1}{\|P_1\|}\sum_{x\in P_1}\min\limits_{y \in P_2}\|x-y \|_{2}^{2} + \frac{1}{\|P_2\|}\sum_{x\in P_2}\min\limits_{y \in P_1}\|x-y \|_{2}^{2}
    \end{equation}



We use Chamfer Distance here to learn sensible particle dynamics $L_{c} =d_c(\hat{P}, P)$, so we can train the differentiable dynamics model using gradient descent. Also, we set a merge loss $L{m}$ to avoid particles from getting too close to each other, we realize the merge loss by penalize the gated distance (gated by $d_{min}$) of nearest neighbor of each particle:

\begin{equation}
\setlength{\abovedisplayskip}{3pt}
    \setlength{\belowdisplayskip}{3pt}
  L_{m} = \sum_{v \in \hat{P}} (ReLU(nd(v) - d_{min}))^2
\end{equation}

where $ nd({v_i}) = \min_{v\in \mathcal{N}(v_i)} d(v_i, v)$. Finally, the loss $L_{dy}$ for training the dynamics model is $L_c + L_m$.

==> text/supp_old.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\appendix

\section{3D point representation from trained pixelNerf}\label{sup-3d-represnetation}

 For a dataset that contains $N_t$ trajectory videos, each video  has $N_f$ frames and each frame is taken from $N_v$ views. Actually we have $N_t * N_f * N_v$ images from $N_{s} = N_t * N_f$ different scenes. We note $\textbf{I}^{(i, j, k)}$ as the image from $i$-th trajectory, $j$-th frame and $k$-th view. We can train a pixelNeRF $F_{\phi}$ on the a subset of the trajectories and it can generalize in other trajectories.

Then for scene $s \in \{1, 2, ..., N_s\}$ with $O_s$ target object(such as fluid, cube), we sample a volumetric space $\textbf{R}(T)$ sized $T * T * T$ in the middle of the desk which can cover the scene and query all the $T^3$ points in the volume to get $(\textbf{c}, \sigma) = F_{\phi}(\textbf{R}(T))$. Then we can select from the $\textbf{R}(T)$ using the density value $\sigma$ to get the point cloud of objects in the scene(container, water, box, robot arm, table): $\textbf{R}_{obj}(T) = \{t \in \textbf{R}(T) | \sigma(t) > \sigma_{min}\}$, where $\sigma_{min}$ is the lowest bar for object density. Here we use color as prior information to segment out the points we want to modeling(water, box). Specifically, for target points which forms a object $o_{i} \in \{1, 2, 3, ..., O_s\}$, we can get the point cloud of this object: $\textbf{R}_{o_{i}}(T) =  \{t \in \textbf{R}_{obj}(T) | \textbf{c}(t) \in r(o_i)\}$ where $r(o_i)$ is the color set for object $o_i$. We note the final point cloud of scene $s$ as $p_{s} = \{p_{s}^{1}, p_{s}^{2}, ..., p_{s}^{O_s}\}$.

Then we can do sparse sampling of each point cloud using FPS (Farthest Point Sampling), which can sample small subset of the target point cloud and maintain the shape of it. To facilitate the learning of particle-based dynamics, we set the size after sampling fixed.


\section{Graph-Based Dynamics Model without Particle-level Correspondence} \label{dpi-wo-correspondece}

As we described in Section 3.2 in the paper, the attributes $a^{v}_{i}$ of a vertex $v_i$ in the built graph includes: 1. velocity of this point in the past frames, 2. attributes of the point (rigid, fluid, granular). To get the velocity of $v$, we should have the history position of $v$. However, since the point-cloud is directly generated from images and do not have particle-level labels. It is hard to get the velocity of one specific points in the graph, since we lack one-to-one correspondence between points. To deal with this problem and make us able to learn complex fluid dynamics without particle-level correspondence, we make small modifications on the original graph-based model in \cite{DPI}.

We assume that we know the dense-labeled states of some known fully-actuated shape like desk and cups that is connected to the robot arms. Here we will list one specific scenario where a cup of water is poured out into another cup. In this case, we have two different types of points: points for fluid and points for cups, we name the states of them in time step $t$ as $V_{P}^{t}=\{v_{P, i}^{t}\}$ and $V_{S}^{t}=\{v_{S, i}^{t}\}$ respectively. For the particle encoder $Q_v$, if the particle belongs to the cups, then the input of particle encoder contains  $n_s$ history states before $t_0$ : $\{V_{S}^{(t_0-n_s):t_0}\}$. If the particle belongs to the water, then we have no history states, so the input of $Q_v$ is all-zero. 


By adding the relative position between receiver and sender points, we can pass the momentum of $V_P$ to $V_S$. Compared with human intuition, we can get an intuitive prediction of the movement of water by simply knowing the past movement of the cup without knowing the past movement of water.




It should also be noted that all the inputs of the dynamics predictor are actually velocity of points or relative position instead of raw position. We do this to make the model translation-invariant so it can be much more generalized when we translate the raw scenario into different scale of coordinate. 



% \section{Online Rolling}

% Online rolling prediction is one of the most significant m


\section{Model Structure of 3D-IntPhys}

Our 3D-IntPhys model can be divided into two parts : one for visual perception, the other for dynamics prediction.

\paragraph{Conditional NeRF} The structure follows that in\cite{pixelnerf}. For the feature encoder in conditional NeRF,  We employ a ResNet34 backbone to extract  feature pyramid by using the feature map prior to the first pooling layer and after the first ResNet 3 layers. Before the training starts, we initialize the weight of feature extractor of the scene using ImageNet pretrained weight. For the NeRF function $f$, We use  fully-connected ResNet
architecture with 5 ResNet blocks with width 512. 

\paragraph{Dynamics Predictor} We use 3-Layer DNN activated by ReLu function with hidden unit sized $150$ for Encoder of both edge and vertex: $Q_e$ and $Q_v$, the propagators $P_e$ and $P_v$ are 1-Layer linear layer followed by ReLU activation, the output dimension of the linear layer is also $150$. 


\paragraph{Sample 3-D Representation} We sample points on a $40 \times 40 \times 40$ grid from an area of $2.5 \text{cm} \times 2.5 cm \times 2.5 cm $ at the center of the table for FluidPour and FluidCubeShake, and on a $70 \times 70 \times 70$ grid from an area of $6 \text{cm} \times 6 cm \times 6 cm $ for GranularPush. We evaluate and include points with a density (measured by the occupancy in the predicted neural radiance fields) larger than $0.99$. Then we subsample the inferred points with FPS with a ratio of around $5\%$ for FluidPour and $10\%$ for FluidCubeShake and GranularPush.


\paragraph{Build Graph} To build graph based on the sub-sampled point-cloud, we set the neighbour distance threshold to be $0.2, 0.15, 0.15$ for FluidPour, FluidCubeShake and GranularPush respectively.


\section{Training Details}


%To train the visual head, we use a learning rate of $1e^{-4}$ with the Adam optimizer. 
%ReduceOnPlateau as the learning rate scheduler.

We sample $64$ points through each ray in the scene to compute the rendering loss when we are training our visual-head. To do paralleling sample from rays, we set the chunk size of NeRF query function $f$ to be $1024*64$.
This can be trained on one RTX-3090 within five hours to get a good visual head perception module that can be used for the following work of point-cloud sampling.


To train our dynamics head, we set batch size to $4$ for all three environments. The learning rate is set to be $1e^{-4}$, using Adam as optimizer. We train the model for $20, 30, 40$ epochs for FluidPour, FluidCubeShake and GranularPush respectively. It takes about $10\sim 15$ hours  to train the dynamics model on one single RTX-3090 for all the three environments.

\section{Dataset Samples}\label{appendix-dataset}

In this section we will give more detailed demonstration of our datasets. Our datasets are generated by NVIDIA Flex in simulation environment, where we can build and scene, add objects and make them move, the relatively accurate physics engine helps us get the movement of points in the scene.  Our dataset focuses on fluid environment, include water, granular and water+cube.

We simulate three kinds of trajectories to represent three basic movement in our daily life: Pour, Shake and Push. Each of the three types (Pour, Shake and Push) has 500 videos of trajectories taken from 6 views, each trajectory has 300 frames.
For each of the three types of video (500 videos), they can be divided into five different settings to make the dataset more diverse. Among these five different settings, the first four of them are regarded as \textbf{interpolate} setting and the last setting is viewed as \textbf{extrapolate} setting. The detailed settings can be referred to in  Table \ref{settings}. Samples from three different kind of envrionments are shown in Figure \ref{pour_sample}, \ref{shake_sample} and \ref{push_sample}. For training-testing separation, we use the separation ratio to be $0.8$, it should be noted that all trajectories for the extrapolate settings are used for testing and will not show up during the training process.

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{imgs/appendix/pour.pdf}
    \caption{Caption}
    \caption{Sample of FluidPour Dataset: the sampling interval is 20 frames, the frames above the blue line are for \textbf{interpolate} data and the other part is for \textbf{extrapolate} data.}
    \label{pour_sample}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{imgs/appendix/shake.pdf}
    \caption{Sample of FluidCubeShake Dataset: the sampling interval is 20 frames, the frames above the blue line are for \textbf{interpolate} data and the other part is for \textbf{extrapolate} data.}
\label{shake_sample}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{imgs/appendix/Push.pdf}
    \caption{Sample of GranularPush Dataset: the sampling interval is 20 frames, the frames above the blue line are for \textbf{interpolate} data and the other part is for \textbf{extrapolate} data.}
\label{push_sample}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[scale=0.4]{imgs/appendix/env_label.png}
    \caption{Labels of container shape referred to in Table \ref{settings}}
    \label{container_shape}
\end{figure}

\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c}
     \hline
    SceneName & Params &   Env1 &  Env2 & Env3 & Env4 & Extrapolate \\
     \hline
     \multirow{7}*{Pour} & X1    & 0  &  0 & 0  & 0 & 0 \\
                         & Y1  & 0  &  0 & 0  & 0  & 0  \\
                         & Z1     & 0  &  0 & 0  & 0  & 0  \\ 
                        & X2     & 0  &  0 & 0  & 0  & 0  \\ 
                        &  Y2      & 0  &  0 & 0  & 0  & 0  \\ 
                        &  Z2      & 0  &  0 & 0  & 0 & 0 \\ 
                        & AmountofWater    & 5125  &  5125 & 6125  & 5375 & 7625 \\
      \hline
      \multirow{4}*{Shake} & X1     & 0  &  0 & 0  & 0  & 0  \\ 
                        &  Y1      & 0  &  0 & 0  & 0  & 0  \\ 
                        &  CubeNumber  & 1  &  1 & 2  & 2 & 3  \\
                        & Water   & 2173  &  3322 & 3322  & 4858 & 4983 \\
      \hline
      \multirow{1}*{Push} & GranularNumber  & 2197  &  4032 & 5832  & 9261 & 12167 \\
                        
      \hline
    \end{tabular}
    \caption{Environment Settings: settings include some basic components of the scene, e.g. shape of container, amount of water, number of cubes. Labels can be referred to in Figure \ref{container_shape}}
    \label{settings}
\end{table}

\begin{figure}
    \centering
    \includegraphics[scale=0.4]{imgs/appendix/seg.png}
    \caption{Example: instance segmentation through color in visual head 3d-pointcloud, red points are ground truth positions}
    \label{fig:my_label}
\end{figure}





\section{More  Qualitative  Results for Visual Head Reconstruction}


\section{More Qualitative Results for Dynamics Prediction}





\section{Potential Society Impact}
\modelname~can be applied to a wide range of down-stream applications, including general scene understanding tasks, robotics manipulation, 3D generative models, and differentiable physics engines. Out work shows the possibility of learning dynamics models from raw sensory inputs, opening up the opportunity to automate the design of differentiable physics engine though data-driven learning algorithms. Predictions from our model is highly interpretable which makes it straightforward to explain model behaviors and re-purpose the outputs for downstream applications. Though data-driven approaches are potentially more scalable, it also brings in the concern that it might be hard to ensure the model behavior to be robust under sensor noise and adversarial attacks, and to fully mitigate data biases. Bringing in advanced technique from ML robustness will be one critical future avenue to pursue.


\subsection{3D point representation from trained perception module}

\begin{figure}[h!]
    \centering
    \includegraphics[width=.8\linewidth]{imgs/appendix/seg.png}
    \caption{
    \textbf{Qualitative Reconstruction and Segmentation Results of the Perception Module.} We show on the left reconstructed 3D shape of the fluid and on the right reconstructed 3D shape of a cube floating in the fluid. Red points are ground truth point positions.}
    \label{fig:my_label}
\end{figure}
% Figure-6 : 

